Optimal Thompson Sampling strategies for support-aware CVaR bandits

In this paper we study a multi-arm bandit problem in which the quality of each arm is measured by the Conditional Value at Risk (CVaR) at some level alpha of the reward distribution. While existing works in this setting mainly focus on Upper Confidence Bound algorithms, we introduce a new Thompson Sampling approach for CVaR bandits on bounded rewards that is flexible enough to solve a variety of problems grounded on physical resources. Building on a recent work by Riou & Honda (2020), we introduce B-CVTS for continuous bounded rewards and M-CVTS for multinomial distributions. On the theoretical side, we provide a non-trivial extension of their analysis that enables to theoretically bound their CVaR regret minimization performance. Strikingly, our results show that these strategies are the first to provably achieve asymptotic optimality in CVaR bandits, matching the corresponding asymptotic lower bounds for this setting. Further, we illustrate empirically the benefit of Thompson Sampling approaches both in a realistic environment simulating a use-case in agriculture and on various synthetic examples.

==> conclusion.tex <==
\section{Conclusion}

The bandit literature where the mean is not the criteria considered to choose between the arms is currently dominated by UCB algorithms. We proposed the first Thompson Sampling approaches for CVaR bandits with \MCVTS{} and \CVTS{}. We gave an upper bound on the CVaR regret of \MCVTS{} and \CVTS{}, showing that these algorithms are \textit{asymptotically optimal} for the set of distributions they tackle, which is the first time such result is proved outside the classical bandit setting. Our experiments demonstrated the interest of our approach to tackle real-world problem with an example in food security. Furthermore, an extensive set of experiments exhibit the benefits of TS approaches over their UCB counterparts. For this reason, we think that this non-parametric way to perform Thompson sampling could be used in other settings, such as the EDPM framework of \citet{cassel}. An interesting future work could be to characterize the set of metrics for which Non-Parameteric Thompson Sampling can work.

\tododo{TODO (choses prioritaires)
\begin{itemize}
	\item Complete section sketch of proof, carefully choose which elements to include
	\item Complete the experiments section
	\item Reorganize the Appendix: Choose their order, which sections to merge etc.
\end{itemize} }

==> introduction.tex <==
\section{Introduction}\label{sec::intro}

A $K$-armed bandit problem is a sequential decision-making problem in which a learner sequentially
samples from $K$ initially unknown distributions $\bm\nu = (\nu_1, \dots, \nu_K)$ called arms. At each time step $t$ a learner chooses an arm
$A_t \in \{1,\dots, K\}$ and collects a random reward $X_t$ drawn from the distribution of the chosen arm, that is $X_t \sim \nu_{A_t}$. 
%that has a cumulative distribution function (CDF) $(F_1, \dots, F_K)$. 
In the classical bandit problem the learner should adjust her sequential sampling strategy $\cA = (A_t)_{t\in \mathbb{N}}$ (or bandit algorithm) in order to maximize the expected total reward obtained after $T$ selections. 
However, in a large number of application domains (healthcare, agriculture, marketing,...) the \textit{expected} reward is not a satisfying measure of the goodness of an arm as it does not reflect well the \textit{preferences} of the learner, and a suitable utility function can be used instead. 
Amongst the various candidate criterion to replace the expectation, the \textit{Conditional Value at Risk} (CVaR) can be a good candidate for the practitioner. Indeed, it depends on a parameter $\alpha \in (0, 1)$ that can model the preferences of the learner, from being neutral to the shape of the distribution ($\alpha\to 1$, classical expectation) to a risk-averse behavior that aim at maximizing the reward in the worst-case scenarios ($\alpha \to 0$). The second case has made CVaR a popular measure in fields such as finance and insurance, at the expense of focusing on specific tools and assumptions to handle extreme risks for (potentially) heavy-tailed distributions.  Those applications are not the focus of our work.
Rather, it is more oriented to applications such as agriculture, healthcare, resource management or marketing, for which CVaR can be a good quality measure for arms without choosing extreme values for the parameter $\alpha$, and even if the distributions are not heavy-tailed. We illustrate this with an example of application in food security in section~\ref{sec::experiments}. In this example, the algorithm recommend planting schemes to farmers. Small holders will usually be more risk-averse than wealthier farmers that are more market-oriented, and hence any value of $\alpha$ could be adapted depending on the nature of the learner. In the sequel we call \textit{CVaR bandits} a bandit problem where the learner wants to maximize the number of times she selects the arm with the largest CVaR.

%The second case has made CVaR a popular measure in fields such as finance and insurance.
%Those applications, however, are not the focus of our work because they are centered on measuring extreme risks for (potentially) heavy-tailed distributions. Our work is instead more oriented to applications such as agriculture, healthcare, resource management or marketing, for which CVaR can be a good quality measure for arms without choosing extreme values for the parameter $\alpha$, and even if the distributions are not heavy-tailed. We illustrate this with an example of application in food security in section~\ref{sec::experiments}. In this example, the algorithm recommend planting schemes to farmers. Small holders will usually be more risk-averse than wealthier farmers that are more market-oriented, and hence any value of $\alpha$ could be adapted depending on the nature of the learner. In the rest of the paper we call \textit{CVaR bandits} a bandit problem where the learner wants to maximize the number of times she selects the arm with the largest CVaR.

Two types of assumptions on the arms's distributions dominate the bandit literature: 1) they belong to a known parametric family (\citet{ HondaTakemura10,Honda15IMED, TS_Emilie, KL_UCB} to name a few), or 2) they are bounded and the bounds are known (e.g \cite{Garivier18KLUCBSwitch, Honda}). In our use-cases the reward distributions are grounded on physical realities, which motivates the use of the second assumption. Indeed, we can realistically assume that the support of the distributions is known and bounded, with bounds that can be  either natural or provided by experts. Secondly, distributions in these settings can have shapes that are not well captured by standard parametric families of distributions, as for instance they can be multi-modal with an unknown number of modes that depend on  external factors unknown at the decision time (weather conditions, illness, pests, \dots). This motivate the design of algorithms that can cover a variety of possible shapes for the distributions. To this purpose, we introduce \CVTS{} for CVaR bandits with \textit{known bounded support}, and \MCVTS{} for CVaR bandits with multinomial arms. We justify the potential use of the two algorithms and their properties in section~\ref{sec::analysis}, and~\ref{sec::experiments}.

Several definitions of the CVaR exist in the literature, depending on whether the samples from the arms are considered as \textit{losses} or as \textit{rewards}. \citet{brown_ineq}, \citet{thomas_concentration} and \citet{agrawal2020optimal} consider the \textit{loss} version of CVaR, defined for any level of risk $\alpha \in (0,1)$ as \[\CVAR_\alpha^-(\nu_k)=\inf_{x \in \R} \left\{x + \frac{1}{\alpha} \bE_{X\sim \nu_k} \left[(X-x)^+\right] \right\}\]
while \citet{galichet2013exploration} and \citet{tamkindistributionally} use the \textit{reward} version of CVaR, defined as \begin{equation}\label{eq::cvar_def}\CVAR_{\alpha}(\nu_k) = \sup_{x \in \R} \left\{x - \frac{1}{\alpha} \bE_{X \sim \nu_k}\left[\left(x-X\right)^+\right] \right\}\;. \end{equation}
We adopt the second definition, which implies that the best arm is the one with the \textit{largest} CVaR. To simplify the notation we write $c_k^\alpha=\CVAR_\alpha(\nu_k)$ in the rest of the paper. 

Following \citet{tamkindistributionally}, we measure the performance of an algorithm using CVaR regret, defined at time $T$ and for some risk-level $\alpha$ as
\begin{align}\cR^{\alpha}_{\bm\nu}(\cA,T)=&\bE_{\bm\nu}\left[\sum_{t=1}^T \left(\max_k c_k^\alpha - c_{A_t}^\alpha \right) \right] \nonumber\\
=& \bE_{\bm\nu}\left[\sum_{t=1}^T \Delta_{A_t}^\alpha \right]= \sum_{k=1}^K \Delta_k^\alpha \bE_{\bm\nu}[N_k(T)],\label{def::regret}\end{align}
where $\Delta_k^\alpha = \max_{k'} c_{k'}^\alpha - c_k^\alpha$ is the gap in CVaR between arm $k$ and the best arm, and $N_k(t) =\sum_{s=1}^{t}\ind(A_s=k)$ is the number of selections of arm $k$ up to round $t$. Other notions of regret have also been studied for risk-averse bandits, some of them computing the risk metric of the full trajectory of observed rewards (e.g., \citet{sani_mv,cassel}). Analyzing such regret can be done when the metric is simple enough (e.g mean-variance) but becomes more complicated when it is not linear and additive, which is the case for CVaR. As noted by \citet{tamkindistributionally}, one of the regret notions studied by \citet{cassel}, called the proxy regret, is an upper bound on the CVaR regret, hence algorithms with guarantees in terms of proxy regret can also serve as baselines in our setting. 

\paragraph{Contributions} Existing algorithms with CVaR regret guarantees are variants of \textit{Upper Confidence Bound} strategies, relying on successive developments of concentration inequalities for the CVaR. 
Building on the work of \citet{Honda}, we propose in this paper a CVaR bandits algorithms based on the \textit{Thompson Sampling} principle. We introduce in Section~ \ref{sec::algorithms} two algorithms: \MCVTS{} for multinomial distributions, and \CVTS{} for continuous distributions with known bounds. 
Unlike previous work on the CVaR, we target in this work \textit{asymptotic optimality}, which has been widely studied in the classical bandit problem but not in this context: We provide in Theorem~\ref{thm:LB} a lower bound on the CVaR regret, highlighting the best achievable problem-dependent performance of a bandit algorithm in this setting. We further show in Theorem~\ref{th::regret_MCVTS} and Theorem~\ref{th::regret_CVTS} that \MCVTS{} and \CVTS{} algorithms are the first to provably match this lower bound for the respective family of distributions they consider. The detailed proof requires non-trivial adaptions for the existing  analysis provided for TS, and especially of one result related to CVAR boundary crossing that required specific focus and is of independent interest.
In Section~\ref{sec::experiments}, we finally consider a use-case in agriculture and highlight the benefits of using the generic Thompson sampling approach in this setting: it gets improved regret compared to UCB algorithms that tend to suffer from non-optimized confidence bounds. Further, its adaptive nature to various families of distributions and simplicity makes it especially relevant for the practitioner.
 We complete this study with experiments on synthetic data that confirm the benefit of Thompson Sampling.



%\paragraph{Contributions} Existing algorithms with CVaR regret guarantees are variants of \textit{Upper Confidence Bound} strategies, relying on successive developments of concentration inequalities for the CVaR. 
%Building on the work of \citet{Honda}, we propose in this paper a CVaR bandits algorithms based on the \textit{Thompson Sampling} principle. We introduce in Section~ \ref{sec::algorithms} two algorithms: \MCVTS{} for multinomial distributions, and \CVTS{} for continuous distributions with known bounds. 
%Unlike previous work on the CVaR, we target in this work \textit{asymptotic optimality}, which has been widely studied in the classical bandit problem but not in this context: We derive the corresponding lower bound on the CVaR regret in Theorem~\ref{thm:LB}. This result is the first to introduce the best possible performance of a bandit algorithm in this setting. We further prove in Theorem~\ref{th::regret_MCVTS} and Theorem~\ref{th::regret_CVTS} that these two algorithms are the first to reaching this lower bound for the family of distributions they consider. Finally, we report in Section~\ref{sec::experiments} a use-case of our algorithms in agriculture and show the benefits of our approach in this setting, compared with the UCB algorithms. We complete this study with experiments on synthetic data that confirms that Thompson Sampling approaches largely outperforms their UCB counterparts.

==> related_work.tex <==
\section{Related work}\label{sec::related}


The Conditional Value at Risk is a well-established statistical measure (see \cite{mandelbrot1997variation}, \citet{artzner} and \citet{acerbi2002coherence}), introduced to formalize mathematically the concept of risk awareness.
 \CVAR{} is a coherent spectral measure in the sense of \citet{rockafellar2000optimization}, as shown in \citet{acerbi2002coherence}), usually considered to be easily interpretable.
 For that reason,  \CVAR{} has been used for a long time by practitioners in fields such as finance (e.g \citet{dowd2007measuring}) thanks to its intuitive definition as the expected reward in the worst $\alpha$-fraction of the outcomes. The study of CVaR in a bandit context is more recent, and is part of a line of works that aim at departing from the idea that the expectation is the best criteria to evaluate an arm. Before considering the specific CVaR bandit literature we first provide a short overview of the bandit literature that led to consider this setting.

\paragraph{Multi-armed bandits} Research on multi-armed bandit has been been shaped by problems where the quality of an arm is measured by its expected value, focusing research efforts on solving the \textit{exploration/exploitation} dilemma (see \citet{Banditbook} for a survey), with great success. Hence, the state-of-art algorithms developed in this setting naturally suggest strategies to handle the CVaR regret. The two most popular approaches are Upper Confidence Bounds (UCB) algorithms (e.g., \citet{agrawal95}, \citet{auer2002finite}, \citet{KL_UCB}) and Thompson Sampling (TS) \cite{TS_1933, TS12AG}. These algorithms are known to have logarithmic regret under yet some stringent assumptions on the arms distributions. 
For example Thompson Sampling strategies are known to be asymptotically optimal when the rewards distributions belong to a one-dimensional exponential family \citep{agrawal13optTS,korda13TSexp}, in that its regret is matching the problem-dependent lower bound on the regret given by \citet{LaiRobbins85}. 
Unfortunately, assuming a simple parametric distributions may not be meaningful to model complex, realistic situations such as the cases we study in this paper. To overcome this limitation, alternative strategies together with strong optimality guarantees have also been derived for more general, possibly non-parametric distribution, targeting the minimal achievable regret given by the lower bound of \citet{burnetas96LB}. The IMED algorithm of \citet{Honda15IMED} and the KL-UCB-Switch algorithm of \citet{Garivier18KLUCBSwitch} are known to match this lower bound for bounded distribution. More recently, \citet{Honda} proposed the first variants of Thompson Sampling strategy having similar properties. 

\paragraph{CVaR bandits} One of the first attempt to depart from the mean in bandits has been the study of the \textit{mean-variance risk} in multi-armed bandit literature (see \citet{sani_mv}, \citet{vakili2}, \citet{vakiliZ16}, \citet{zimin_ra}). On the other hand, \cite{szorenyi2015qualitative} considered
a quantile-based bandit approach (hence focusing on the Value-at-Risk) in both cumulated regret minimization and best arm identification setting, while, the \textit{entropic risk} were studied by \citet{oda_raucb}.
In a recent work \citet{cassel} studied a general class of problems under the \textit{empirical distribution performance metric} (EDPM) framework, that captures the previous settings as well as spectral risk measures such as the CVaR. 
It is worth noting that all the strategies studied in these papers are UCB strategies.
On the other hand, the first Thompson Sampling algorithm was proposed by \citet{MVTS} for the mean-variance criterion. The recent work of \citet{chang2020riskconstrained} explores an extension of Gaussian Thompson Sampling to the related \textit{risk-constrained setting} introduced by \citet{kagrecha20riskconstrained}, in which the goal is to maximize the mean rewards under the constraint that arms with a small \CVAR{} are not played too often. This works in interesting as it shows that Thompson Sampling in parametric families can be extended to CVaR, but is unfortunately restricted to the specific case of Gaussian bandits.

Strategies following the optimism principle are dominant in the literature specific to CVaR bandits. In order to build such a strategy, one requires concentration inequalities on the considered risk metric. 
Two main approaches can be distinguished: adding a bonus to an empirical metric as considered in \citet{galichet2013exploration,galichet2015contributions, cassel}  or directly computing an optimistic empirical CDF as in \cite{tamkindistributionally}. At the heart of these approaches is the Dvoretzky--Kiefer--Wolfowitz (DKW) concentration inequality (see \citet{massart1990}), a fundamental result which provides exponential concentration bound on the probability that an empirical CDF deviates from its true CDF. This inequality has been used for example by \citet{brown_ineq} and \citet{thomas_concentration} to develop concentration inequalities for the empirical \CVAR{} of bounded distributions. These results lead different authors to design different UCB algorithms for CVaR bandits with bounded rewards: MaRaB \cite{galichet2013exploration}, U-UCB \cite{cassel}, and \CVAR-UCB \cite{tamkindistributionally}. 

\begin{remark}
In this paper we compare our proposed algorithms with U-UCB and \CVAR-UCB. MaRaB is similar to U-UCB but studied under a more limited theoretical setting, with weaker guarantees, hence is excluded from our experiments. Also, \citet{cassel} gives an upper bound on the proxy regret of U-UCB, which hence is also valid for the smaller CVaR regret. For completeness, we provide in Appendix~\ref{app::brown_ucb} an analysis of U-UCB specifically tailored to the CVaR regret, and also discuss its links with the Brown-UCB approach of \citet{tamkindistributionally}.
\end{remark}
		

Recent works have proposed concentration inequalities for the empirical CVaR of unbounded distributions under non-parametric assumptions \citep{KagrechaNJ19,cvar_conc_prashanth,holland2020learning}, yet under some debatable assumptions. For instance \cite{cvar_conc_prashanth} requires knowledge of a specific lower bound on the pdf around the quantile at given risk level, which is often unknown ot the practitioner. Such results could be used to derive UCB algorithms for specific heavy-tailed distributions, but provide little insights on to design and analysis of a general Thompson Sampling algorithm designed to be asymptotically optimal in a variety of cases.

\tododo{Je trouve ce dernier paragraphe peut-être un peu "aggressif". C'est peut-être que je francise le sens du mot "debatable" (j'ai traduit par "discutable" dans ma tête, qui est assez péjoratif), mais je préfère te demander confirmation.}
%Restricting our attention to bounded distributions, we propose the first Thompson Sampling algorithms tailored to minimizing the CVaR regret. 

Finally, we mention that CVaR bandits have also recently been studied under the different pure exploration setting \citep{KagrechaNJ19,agrawal2020optimal}.


\oam{Add litterature on extreme bandits to say it is rather different perspective ? }

\paragraph{Baselines and contributions} We compare both U-UCB and CVaR-UCB to the algorithms we introduced as they showcase two fundamentally different approaches to build a UCB strategy for a non-linear utility function. The first consists in adding a confidence bonus to the empirical value of the metric, while the second  computes the metric for an \textit{optimistic version of the distribution}. The first method is closely related to UCB approaches in the classical bandit setting, while the second tries to capture the properties of the underlying CDF and may be generalized to different risk metrics without changing the bonus. \citet{tamkindistributionally} claim the superiority of this second approach, and our experimental results seem to confirm it. On the theoretical side, both U-UCB and CVaR-UCB provably achieve a logarithmic CVaR regret in bandit models with bounded distributions, with a scaling in $\frac{K\log T}{\alpha^2 \Delta}$ where $\Delta$ is the smallest (positive) CVaR gap $\Delta_k^{\alpha}$. However, the asymptotic optimality has not been studied in the CVaR literature and it has not been established so far that the scaling of these bounds is near-optimal. We derive a lower bound on the CVaR regret in Theorem~\ref{thm:LB}, suggesting that the analysis of these algorithms make appear a gap and hence may not ensure asymptotic optimally.  In Section~\ref{sec::algorithms} we introduce two algorithms, one for multinomial and one for bounded distributions, that are aimed at matching the lower bound derived in Theorem~\ref{thm:LB}. We prove in Section~\ref{sec::analysis} their asymptotic optimality in Theorem~\ref{th::regret_MCVTS} and Theorem~\ref{th::regret_CVTS}. Up to our knowledge, these results are the first showing asymptotic optimality of a TS based CVaR regret minimization strategy.

